Sustainability is Stratified: Toward a Better Theory of Sustainable Software Engineering

Background: Sustainable software engineering (SSE) means creating software in a way that meets present needs without undermining our collective capacity to meet our future needs. It is typically conceptualized as several intersecting dimensions or ``pillars'' -- environmental, social, economic, technical and individual. However; these pillars are theoretically underdeveloped and require refinement. Objectives: The objective of this paper is to generate a better theory of SSE. Method: First, a scoping review was conducted to understand the state of research on SSE and identify existing models thereof. Next, a meta-synthesis of qualitative research on SSE was conducted to critique and improve the existing models identified. Results: 961 potentially relevant articles were extracted from five article databases. These articles were de-duplicated and then screened independently by two screeners, leaving 243 articles to examine. Of these, 109 were non-empirical, the most common empirical method was systematic review, and no randomized controlled experiments were found. Most papers focus on ecological sustainability (158) and the sustainability of software products (148) rather than processes. A meta-synthesis of 36 qualitative studies produced several key propositions, most notably, that sustainability is stratified (has different meanings at different levels of abstraction) and multisystemic (emerges from interactions among multiple social, technical, and sociotechnical systems). Conclusion: The academic literature on SSE is surprisingly non-empirical. More empirical evaluations of specific sustainability interventions are needed. The sustainability of software development products and processes should be conceptualized as multisystemic and stratified, and assessed accordingly.

==> TODO.tex <==

- finish the data extraction spreadsheet and upload it to Figshare. Make sure the address to the replication package in the paper is still correct. - SEAN (DEC 19) Done
- update the jupyter notebook, add it to figshare and refresh figs - SEAN (DEC 19) 
- the full citations of the core result set in the paper - ERIN (DEC 19) - Done
- update all the numbers on overleaf (e.g. numbers of primary studies) including table II - ERIN (DEC 19) - mostly done, just waiting on a couple of new figs
- a revision (or removal) of the diagram - PAUL DONE
- a detailed characterization of stratification as outlined in response 2 - PAUL DONE
- fix all minor errors mentioned by reviews - BIMPE (DEC 19)
- Look at the one paper that could be added to the synthesis and see how to fit it in somewhere: How Could We Have Known? Anticipating Sustainability Effects of a Software Product - BIMPE (DEC 19)


Summary of How Could We Have Known? Paper
The authors conducted a case study to show how the Sustainability Awareness Framework (SusAF) can be applied to identify the potential sustainability effects of an IT company’s (software) product.

The paper fits into proposition 1, since the aim of the case study was to identify the sustainability effects of the company’s financial management software. Before the case study, the company recognized only three sustainability effects that their financial management software might have, but with the Sustainability Awareness Framework (SusAF), 28 direct (first-order) effects, approx 100 enabling (second-order) effects and 23 structural (third-order) effects and several chains of effects, which were finally grouped into six high-level categories were identified. 

The authors also cited examples of how the different effects relates to sustainability.



==> tables/processExamples.tex <==
\begin{table*}[t]
\centering
\caption{Examples of each sustainability dimension for software development processes}
\label{tab:tab_processExamples}
\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{\linewidth}{lXX} %this makes a table the width of the page or column that has two equal-width, autoresizing columns. We can manually adjust the column width if necessary right before submitting.
\toprule
\textbf{Dimension} & \textbf{Helps} & \textbf{Harms} \\ 
\midrule
Ecological & A software company introduces a “green” policy to reduce the carbon footprint of their offices. & A startup opens a crypto-mining warehouse, leading to a huge increase in the company's electricity usage. \\
Social & A software team holds monthly hackathons to help its members bond and collaborate on fun projects together. & A software company promotes overwork by expecting developers to work evenings and weekends, leading to high turnover and knowledge loss between developers. \\
%Individual & A software company recognizes the achievements of a senior developer by offering a higher salary and a leadership role. & A company fosters a culture of overwork where employees are expected work evenings and weekends regularly  \\
Economic & Instead of writing new code, a company reduces costs by building their website with a free, open-source framework. & When a software company misses another deadline, their client decides to hire a different company for the project. \\
\bottomrule
\end{tabularx}
\end{table*}



==> tables/productExamples.tex <==
\begin{table*}[t]
\centering
\caption{Examples of each sustainability dimension for software products}
\label{tab:tab_productExamples}
%\renewcommand{\arraystretch}{1.3} %you don't have to set this for every table. It'll just keep using the value you set in the last table environment
\begin{tabularx}{\linewidth}{lXX}
\toprule
\textbf{Dimension} & \textbf{Helps} & \textbf{Harms} \\
\midrule
Ecological & An application update is released that consumes significantly less energy than previous versions. & A new mobile phone OS renders previous hardware obsolete, producing large amounts of waste. \\
Social & A city creates a digital museum app, allowing free access to the city's art and historical resources. & A social media application shows controversial content, leading to aggression and discourse between users. \\
%Individual & A website for independent creators chooses a new creator to highlight on their front page each week, leading to more exposure and opportunities for those selected. & Deepfake technology is used to create fake embarrassing videos of a public speaker, damaging their reputation. \\
Economic & A gaming company adds microtransactions to their game, allowing a steady stream of revenue for each copy sold. & An ad-supported website accidentally has a security leak, causing many users to leave permanently. \\
Technical & A content-blocking extension uses machine learning to identify harmful content, allowing it to grow over time. & A web app relies heavily on several open-source dependencies and stops working when one of them become defunct. \\
\bottomrule
\end{tabularx}
\end{table*}
